Approximate NNLO Predictions for the Stop-Pair Production Cross Section at the LHC

If the minimal supersymmetric standard model at scales of around 1 TeV is realized in nature, the total top-squark pair production cross section should be measurable at the CERN Large Hadron Collider. In this work we present precise predictions for this observable, which are based upon approximate NNLO formulas obtained using soft-collinear effective theory methods.

==> programs/Fortran/mymathlib/makefile <==
LIB = ../libmymathlib.a

OBJS = \
mtlprt.o \
dilog64.o \
cgplg64.o

$(LIB): $(LIB)($(OBJS))
	ranlib $(LIB)

%.o: %.f
	$(F77) $(F77FLAGS) -c $<

clean:
	$(RM) *.o



==> programs/Fortran/prospino/makefile <==
LIB = ../libprospino.a

OBJS = \
matrixst.o \
integral.o \
integralst.o \
hadronst.o \
prospino_interface.o

$(LIB): $(LIB)($(OBJS))
	ranlib $(LIB)

%.o: %.f
	$(F77) $(F77FLAGS) -c $<

clean:
	$(RM) *.o


